A First Step Towards Understanding Real-world Attacks on IoT Devices

With the rapid growth of Internet of Things (IoT) devices, it is imperative to proactively understand the real-world cybersecurity threats posed to them. This paper describes our initial efforts towards building a honeypot ecosystem as a means to gathering and analyzing real attack data against IoT devices. A primary condition for a honeypot to yield useful insights is to let attackers believe they are real systems used by humans and organizations. IoT devices pose unique challenges in this respect, due to the large variety of device types and the physical-connectedness nature. We thus create a multiphased approach in building a honeypot ecosystem, where researchers can gradually increase a low-interaction honeypot's sophistication in emulating an IoT device by observing real-world attackers' behaviors. We deployed honeypots both on-premise and in the cloud, with associated analysis and vetting infrastructures to ensure these honeypots cannot be easily identified as such and appear to be real systems. In doing so we were able to attract increasingly sophisticated attack data. We present the design of this honeypot ecosystem and our observation on the attack data so far. Our data shows that real-world attackers are explicitly going after IoT devices, and some captured activities seem to involve direct human interaction (as opposed to scripted automatic activities). We also build a low interaction honeypot for IoT cameras, called Honeycamera, that present to attackers seemingly real videos. This is our first step towards building a more comprehensive honeypot ecosystem that will allow researchers to gain concrete understanding of what attackers are going after on IoT devices, so as to more proactively protect them.

==> Makefile <==
.PHONY: all clean paper

all:  paper 
#\
#    tikz/storage-traditional.pdf \
#    tikz/storage-disaggregated.pdf \
#    tikz/storage-disaggregated-ops.pdf \
#    tikz/ebpf-data.pdf \
#    paper

tikz/%.pdf: tikz/%.tex
	xelatex -output-directory=tikz/ $<
	pdfcrop $@

paper:
	latex-mk --pdflatex main.tex || true


==> section4.tex <==
\section{Multi-faceted and multi-phased deployment/experimentation}
\label{sec:multiphased}

%\hspace{\parindent}
For the purpose of this project, a multi-faceted approach was chosen.  Although, these honeypots provided satisfactory results, to have more specific information on IoT attacks, {\it HoneyCamera} designed and deployed along with others. Each one of these honeypots emulated at least one IoT device’s protocol, including {\it HTTP} and {\it SSH}, to name just two.
In addition, honeypots were deployed in different phases. The first phase had the least changes from the original software to start receiving attacks. From this point, honeypot ecosystem started to collect data, and the analyzed data helped to create the subsequent phase by understanding what cybercriminals are looking for, and how this ecosystem can become more sophisticated. The second phase was repeated many times until acceptable results were achieved. At the end, in phase three, previous information was used to create more advanced low interaction honeypots. In this section, these taken approaches are presented.

\begin{description}
\item[HoneyLogin] Cowrie honeypot was used to emulate a vulnerable IoT device with open SSH (port 22) or telnet (port 23). Three main honeypots' instances were created in three different phases, and Busybox OS was also picked for this purpose.
\begin{itemize}
  \item In the first phase, the system was allowed to accept every possible combination of usernames and passwords. Two honeypots were implemented, one in Singapore and the other one inside the university’s infrastructure.
  \item In the second phase which started after 6 months, the top 30 username/password combinations were picked with command execution to create a new honeypot instance inside the university's network. In addition, new usernames and file systems were created, and more bait was added to it. Accordingly, previous logs were analyzed, and all of the problems encountered in the first phase were fixed, such as \textit{file} command's response added to the honeypot configuration.
  \item In the last phase, all the information collected was used to create a more sophisticated honeypot. As a result, a complex password was generated, and the number of possible successful login combinations was limited to only one. Since the password was set to be very complicated, every successful login would imply that it was possibly done by a real hacker which consequently could provide valuable information.
\end{itemize}

\item[HoneyWindowsBox] Dionaea was the second installed honeypot for this purpose.
\begin{itemize}
\item In the first phase, a default version of Dionaea was installed through cloud infrastructure. Unfortunately, this version could not pass the vetting system and was easily found as a honeypot.
\item To achieve a hard detectable honeypot, in phase two, services were broken down into two different combinations. The first honeypot had FTP, HTTP and HTTPS services while only SMB and MSSQL services were enabled for the second one. Three locations were chosen to install Dionaea (India, Canada and the university's network). These IPs popped up as a real system in Shodan. KFSensor honeypot was the second honeypot that was installed during this step. For this purpose, an educational license was acquired from Keyfocus. Paris and the United States were chosen as the locations to install this honeypot.
\end{itemize}
\item[HoneyCamera] is the last implemented honeypot. Different cameras have different available ports.
\begin{itemize}
\item In the first phase, three honeypots were implemented. Two servers in Sydney and Paris had only port 8080 exposed while the other one in London had port 80. The first Two Honeypots were used to emulate D-Link DCS-5020L and the other one to imitate D-Link DCS-5030L camera.
\item In the second phase, a combination of HoneyCamera and HoneyLogin will be implemented. At this time, this process is still under development.
\end{itemize}
\end{description}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

